Optimizing Temporal Convolutional Network inference on FPGA-based accelerators

Convolutional Neural Networks are extensively used in a wide range of applications, commonly including computer vision tasks like image and video classification, recognition, and segmentation. Recent research results demonstrate that multilayer(deep) networks involving mono-dimensional convolutions and dilation can be effectively used in time series and sequences classification and segmentation, as well as in tasks involving sequence modelling. These structures, commonly referred to as Temporal Convolutional Networks (TCNs), have been demonstrated to consistently outperform Recurrent Neural Networks in terms of accuracy and training time [1]. While FPGA-based inference accelerators for classic CNNs are widespread, literature is lacking in a quantitative evaluation of their usability on inference for TCN models. In this paper we present such an evaluation, considering a CNN accelerator with specific features supporting TCN kernels as a reference and a set of state-of-the-art TCNs as a benchmark. Experimental results show that, during TCN execution, operational intensity can be critical for the overall performance. We propose a convolution scheduling based on batch processing that can boost efficiency up to 96% of theoretical peak performance. Overall we can achieve up to 111,8 GOPS/s and power efficiency of 33,9 GOPS/s/W on an Ultrascale+ ZU3EG (up to 10x speedup and 3x power efficiency improvement with respect to pure software implementation).

==> Efficiency_batch_size_.tex <==
\resizebox{.8\columnwidth}{.8\columnwidth}{\begin{tikzpicture}
\begin{axis}[
    title={Efficiency to batch size trend for layers of \cite{ecg}},
    xlabel={Batch Size},
    ylabel={efficiency},
    xmin=0, xmax=370,
    ymin=0, ymax=1,
    xtick={0,25,50,75,100,150,200,250,300,350,400},
    ytick={0,0.1,0.2,0.3,0.4,0.5,0.6,0.7,0.8,0.9,1.0},
    legend pos=south east,
    ymajorgrids=true,
    grid style=dashed,
]
 
\addplot[
    color=blue,
    mark=,
    ]
    coordinates {
    (0,0.11)(24,0.756)(192,0.95)(348,0.968)
    };
    \addlegendentry{1\textsuperscript{st} layer}
    
\addplot[
    color=red,
    mark=,
    ]
    coordinates {
    (0,0.058)(24,0.465)(192,0.79)(348,0.85)
    };
    \addlegendentry{2\textsuperscript{nd} layer}
    
\addplot[
    color=green,
    mark=,
    ]
    coordinates {
    (0,0.106)(24,0.738)(192,0.946)(348,0.966)
    };
    \addlegendentry{3\textsuperscript{rd} layer}
    
\addplot[
    color=orange,
    mark=,
    ]
    coordinates {
    (0,0.08)(24,0.545)(192,0.857)(348,0.906)
    };
    \addlegendentry{4\textsuperscript{th} layer}
    
\addplot[
    color=black,
    mark=,
    ]
    coordinates {
    (0,0.064)(24,0.427)(192,0.797)(348,0.86)
    };
    \addlegendentry{5\textsuperscript{th} layer}
    
\addplot[
    color=violet,
    mark=,
    ]
    coordinates {
    (0,0.0648)(24,0.427)(192,0.798)(348,0.858)
    };
    \addlegendentry{6\textsuperscript{th} layer}
    
\addplot[
    color=brown,
    mark=,
    ]
    coordinates {
    (0,0.046)(24,0.31)(192,0.697)(348,0.79)
    };
    \addlegendentry{7\textsuperscript{th} layer}
    
\addplot[
    color=purple,
    mark=,
    ]
    coordinates {
    (0,0.0325)(24,0.216)(192,0.582)(348,0.683)
    };
    \addlegendentry{8\textsuperscript{th} layer}
 
\end{axis}
\end{tikzpicture}
}

==> biblio_item.tex <==
\begin{thebibliography}{99}
\bibitem{bai2018empirical}
Bai, Shaojie, J. Zico Kolter, and Vladlen Koltun. "An empirical evaluation of generic convolutional and recurrent networks for sequence modeling." arXiv preprint arXiv:1803.01271 (2018).

\bibitem{ecg}
Goodfellow, S. D., Goodwin, A., Greer, R., Laussen, P. C., Mazwi, M., \& Eytan, D. (2018, November). Towards Understanding ECG Rhythm Classification Using Convolutional Neural Networks and Attention Mappings. In Machine Learning for Healthcare Conference (pp. 83-101).

\bibitem{humanActRecMobile}
Zeng, M., Nguyen, L. T., Yu, B., Mengshoel, O. J., Zhu, J., Wu, P., \& Zhang, J. (2014, November). Convolutional neural networks for human activity recognition using mobile sensors. In 6th International Conference on Mobile Computing, Applications and Services (pp. 197-205). IEEE.

\bibitem{3D_gesture_class}
Duffner, S., Berlemont, S., Lefebvre, G., \& Garcia, C. (2014, May). 3D gesture classification with convolutional neural networks. In 2014 IEEE International Conference on Acoustics, Speech and Signal Processing (ICASSP) (pp. 5432-5436). IEEE.

\bibitem{humanActRec}
Yang, J., Nguyen, M. N., San, P. P., Li, X. L., \& Krishnaswamy, S. (2015, June). Deep convolutional neural networks on multichannel time series for human activity recognition. In Twenty-Fourth International Joint Conference on Artificial Intelligence.

\bibitem{Ackermann}
Ackermann, Introduction to 1D Convolutional Neural Networks in Keras for Time Sequences. \url{https://blog.goodaudience.com/introduction-to-1d-convolutional-neural-networks-in-keras-for-time-sequences-3a7ff801a2cf}

\bibitem{ecg_class_1D}
Li, D., Zhang, J., Zhang, Q., \& Wei, X. (2017, October). Classification of ECG signals based on 1D convolution neural network. In 2017 IEEE 19th International Conference on e-Health Networking, Applications and Services (Healthcom) (pp. 1-6). IEEE.

\bibitem{3D_skeleton}
Kim, T. S., \& Reiter, A. (2017, July). Interpretable 3d human action analysis with temporal convolutional networks. In 2017 IEEE Conference on Computer Vision and Pattern Recognition Workshops (CVPRW) (pp. 1623-1631). IEEE.

\bibitem{wavenet}
Oord, A. V. D., Dieleman, S., Zen, H., Simonyan, K., Vinyals, O., Graves, A., ... \& Kavukcuoglu, K. (2016). Wavenet: A generative model for raw audio. arXiv preprint arXiv:1609.03499.

\bibitem{polyWaveNet}
Martak, L. S., Sajgalik, M., \& Benesova, W. (2018, June). Polyphonic Note Transcription of Time-Domain Audio Signal with Deep WaveNet Architecture. In 2018 25th International Conference on Systems, Signals and Image Processing (IWSSIP) (pp. 1-5). IEEE.

\bibitem{neu2017}
Meloni, P., Capotondi, A., Deriu, G., Brian, M., Conti, F., Rossi, D., ... \& Benini, L. (2018). NEURA ghe: Exploiting CPU-FPGA Synergies for Efficient and Flexible CNN Inference Acceleration on Zynq SoCs. ACM Transactions on Reconfigurable Technology and Systems (TRETS), 11(3), 18.

\bibitem{img_rec_He_Zhang}
He, K., Zhang, X., Ren, S., \& Sun, J. (2016). Deep residual learning for image recognition. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 770-778).

\bibitem{imagenet_Krizhevsky}
Krizhevsky, A., Sutskever, I., \& Hinton, G. E. (2012). Imagenet classification with deep convolutional neural networks. In Advances in neural information processing systems (pp. 1097-1105).

\bibitem{face_det}
Taigman, Y., Yang, M., Ranzato, M. A., \& Wolf, L. (2014). Deepface: Closing the gap to human-level performance in face verification. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 1701-1708).

\bibitem{yolo}
Redmon, J., Divvala, S., Girshick, R., \& Farhadi, A. (2016). You only look once: Unified, real-time object detection. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 779-788).

\bibitem{lang_model}
Dauphin, Y. N., Fan, A., Auli, M., \& Grangier, D. (2017, August). Language modeling with gated convolutional networks. In Proceedings of the 34th International Conference on Machine Learning-Volume 70 (pp. 933-941). JMLR. org.

\bibitem{lstmFPGA}
Guan, Y., Yuan, Z., Sun, G., \& Cong, J. (2017, January). FPGA-based accelerator for long short-term memory recurrent neural networks. In 2017 22nd Asia and South Pacific Design Automation Conference (ASP-DAC) (pp. 629-634). IEEE.

\bibitem{deepSpeech}
Hannun, A., Case, C., Casper, J., Catanzaro, B., Diamos, G., Elsen, E., ... \& Ng, A. Y. (2014). Deep speech: Scaling up end-to-end speech recognition. arXiv preprint arXiv:1412.5567.

\bibitem{deepImage}
Wu, R., Yan, S., Shan, Y., Dang, Q., \& Sun, G. (2015). Deep image: Scaling up image recognition. arXiv preprint arXiv:1501.02876.

\bibitem{deepFace}
Taigman, Y., Yang, M., Ranzato, M. A., \& Wolf, L. (2014). Deepface: Closing the gap to human-level performance in face verification. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 1701-1708).

\bibitem{videoClass}
Karpathy, A., Toderici, G., Shetty, S., Leung, T., Sukthankar, R., \& Fei-Fei, L. (2014). Large-scale video classification with convolutional neural networks. In Proceedings of the IEEE conference on Computer Vision and Pattern Recognition (pp. 1725-1732).

\bibitem{sentClass}
Kim, Y. (2014). Convolutional neural networks for sentence classification. arXiv preprint arXiv:1408.5882.

\bibitem{textUnde}
Weston, J. E. (2016). Dialog-based language learning. In Advances in Neural Information Processing Systems (pp. 829-837).

\bibitem{NLP}
Santos, C. D., \& Zadrozny, B. (2014). Learning character-level representations for part-of-speech tagging. In Proceedings of the 31st International Conference on Machine Learning (ICML-14) (pp. 1818-1826).

\bibitem{machineTras}
Kalchbrenner, N., Espeholt, L., Simonyan, K., Oord, A. V. D., Graves, A., \& Kavukcuoglu, K. (2016). Neural machine translation in linear time. arXiv preprint arXiv:1610.10099.

\bibitem{deeplearningbook}
Goodfellow, I., Bengio, Y., \& Courville, A. (2016). Deep learning. MIT press.

\bibitem{lstm}
Hochreiter, S., \& Schmidhuber, J. (1997). Long short-term memory. Neural computation, 9(8), 1735-1780.

\bibitem{gru}
Cho, K., Van Merriënboer, B., Bahdanau, D., \& Bengio, Y. (2014). On the properties of neural machine translation: Encoder-decoder approaches. arXiv preprint arXiv:1409.1259.

\bibitem{survey}
Mittal, S. (2018). A survey of FPGA-based accelerators for convolutional neural networks. Neural computing and applications, 1-31.

\bibitem{dlau}
Wang, C., Gong, L., Yu, Q., Li, X., Xie, Y., \& Zhou, X. (2016). DLAU: A scalable deep learning accelerator unit on FPGA. IEEE Transactions on Computer-Aided Design of Integrated Circuits and Systems, 36(3), 513-517.


%\end{thebibliography}


\end{thebibliography}

